KORGym: A Dynamic Game Platform for LLM Reasoning Evaluation

Recent advancements in large language models (LLMs) underscore the need for more comprehensive evaluation methods to accurately assess their reasoning capabilities. Existing benchmarks are often domain-specific and thus cannot fully capture an LLM's general reasoning potential. To address this limitation, we introduce the Knowledge Orthogonal Reasoning Gymnasium (KORGym), a dynamic evaluation platform inspired by KOR-Bench and Gymnasium. KORGym offers over fifty games in either textual or visual formats and supports interactive, multi-turn assessments with reinforcement learning scenarios. Using KORGym, we conduct extensive experiments on 19 LLMs and 8 VLMs, revealing consistent reasoning patterns within model families and demonstrating the superior performance of closed-source models. Further analysis examines the effects of modality, reasoning strategies, reinforcement learning techniques, and response length on model performance. We expect KORGym to become a valuable resource for advancing LLM reasoning research and developing evaluation methodologies suited to complex, interactive environments.

==> tables/Control,_Interaction,_and_Task_Reasoning.tex <==
\begin{table}[h]
    \centering
    \small
    % \renewcommand{\arraystretch}{1.2}
    \resizebox{0.99\textwidth}{!}{
    \begin{tabular}{llp{18cm}}
        \toprule
        No. & Name & Task Content \\
        \midrule
        6 & Minigrid & Based on the Minigrid \citep{MinigridMiniworld23} reinforcement learning system, a control environment tailored for LLMs is constructed, where an agent (ball) performs complex tasks in a partially observable maze, such as picking up items, placing items, avoiding lava, and opening doors.  \\
        18 & Snake & This game tests an LLM’s ability to control a growing snake on a bounded grid, avoiding collisions while strategically navigating toward apples to maximize score.\\
        19 & Tetris & This game tests an LLM’s ability to reason spatially and plan ahead by strategically rotating and placing Tetris blocks to clear rows and maximize the score under dynamic constraints.\\
        32 & Minesweeper & This game tests an LLM’s ability to reason about probabilistic information and spatial patterns by uncovering safe cells and flagging hidden mines on a grid-based board through logical deduction.\\
        35 & PVZ & This game tests an LLM’s ability to optimize resource management and strategic defense by placing plants with diverse effects to counter increasingly strong waves of zombies over time.\\
        41 & Long Cat & This game tests an LLM’s ability to plan efficient movement sequences by navigating a sliding cat to fill all empty spaces on a grid while avoiding obstacles.\\
        42 & Black White Copy & This game tests an LLM’s ability to apply strategic operations on a chessboard by toggling rows, columns, and diagonals to transform an all-white board into a specified black-and-white target pattern within a limited number of moves.\\
        \bottomrule
    \end{tabular}
    }
    \caption{Game Introduction of Control, Interaction, and Task Reasoning}
    \label{tab:task_control}
\end{table}


==> tables/Language_and_Textual_Reasoning.tex <==
\begin{table}[h]
    \centering
    \small
    % \renewcommand{\arraystretch}{1.2}
    \resizebox{0.99\textwidth}{!}{
    \begin{tabular}{llp{18cm}}
        \toprule
        No. & Name & Task Content\\
        \midrule
        2  & word problem & This game challenges an LLM to find a specific English word that matches given letter and length constraints through logical reasoning.\\
        15 & Alphabetical Sorting & In this game, LLM is given an anagram with the first letter fixed, and its task is to rearrange the remaining letters to form a valid word.\\
        16 & Letter Connection & This game tests an LLM’s ability to trace, recognize, and reconstruct a hidden word from a 3x3 letter grid by identifying valid sequential paths.\\
        22 & Word Transformation & This game tests an LLM’s ability to decode a transformed word by reasoning through layered transformations including repetition, shifts, reversals, and emoji mappings.\\
        27 & Wordle & This game tests an LLM’s ability to perform deductive reasoning through iterative word guessing based on structured feedback.\\
        30 & Crypto Word & This game challenges an LLM’s ability to decode a sentence by mapping emojis to letters using frequency analysis and iterative feedback-based guessing.\\
        \bottomrule
    \end{tabular}
    }
    \caption{Game Introduction of Language and Textual Reasoning}
    \label{tab:task_language}
\end{table}


==> tables/Multimodal_Reasoning.tex <==
\begin{table}[h]
    \centering
    \small
    % \renewcommand{\arraystretch}{1.2}
    \resizebox{0.99\textwidth}{!}{
    \begin{tabular}{llp{18cm}}
        \toprule
        No. & Name & Task Content\\
        \midrule
        43 & Crossword Puzzle & This game tests an LLM’s multimodal reasoning ability by interpreting visual information from a crossword puzzle image and solving linguistic clues to correctly fill the grid with words. \\
        44 & Jigsaw Puzzle & This game tests an LLM’s multimodal reasoning and spatial arrangement skills by matching visual puzzle pieces with numbered slots to accurately reconstruct an image.\\
        45 & Find The Pattern & This game evaluates an LLM’s multimodal perception and pattern recognition ability by identifying the correct visual piece that completes a given pattern.\\
        46 & Circle The Cat (Visual) & This game evaluates an LLM’s multimodal reasoning, spatial reasoning and strategic planning by requiring it to analyze a visual board and determine optimal wall placements to prevent a cat from escaping through exits.\\
        47 & Map Simulation (Visual) & This game tests an LLM’s multimodal reasoning, dynamic spatial awareness, and sequential decision-making by interpreting complex visual elements on a map, interacting with diverse objects (portals, traps, jumpers), and accurately calculating the final position of the player based on a series of directional moves.\\
        48 & Sokoban (Visual) & This game tests an LLM’s multimodal problem-solving and sequential reasoning abilities by interpreting a visual Sokoban puzzle and generating a precise series of moves to push all boxes into their designated target areas while respecting spatial constraints and movement rules.\\
        49 & Bubble Ball Sorting (Visual) & This game tests an LLM’s multimodal visual reasoning and strategic planning skills by interpreting a visual tube-and-ball arrangement and generating valid moves to achieve uniform color sorting across specified tubes.\\
        50 & Wordle (Visual) & This game tests an LLM’s multimodal interpretation and linguistic reasoning by analyzing visual feedback from color-coded guesses to deduce the correct five-letter secret word.\\
        51 & Square Addition (Visual) & This game tests an LLM’s multimodal reasoning and numerical deduction by interpreting color-coded patterns in a grid and inferring integer values to compute accurate column sums.\\
        \bottomrule
    \end{tabular}
    }
    \caption{Game Introduction of Multimodal Reasoning}
    \label{tab:task_multimodal}
\end{table}


==> tables/Spatial_and_Geometric_Reasoning.tex <==
\begin{table}[h]
    \centering
    \small
    % \renewcommand{\arraystretch}{1.2}
    \resizebox{0.99\textwidth}{!}{
    \begin{tabular}{llp{18cm}}
        \toprule
        No. & Name & Task Content\\
        \midrule
        7 & Maze & This game challenges an LLM to find a valid path through a maze from the start point 'I' to the destination 'X', avoiding walls and outputting the sequence of moves. \\
        8 & Sokoban & This game tests an LLM's planning ability by requiring it to solve a Sokoban puzzle, pushing all boxes onto target areas while navigating walls and obeying movement constraints. \\
        9 & Playlines & This game tests an LLM’s ability to solve a path-finding and filling puzzle by connecting identical numbers on a grid without leaving empty spaces or branching.\\
        10 & Emoji Connect & This game tests an LLM’s ability to analyze structured emoji grids by identifying and counting repeated horizontal or vertical patterns based on simple adjacency rules.\\
        17 & 8-puzzle & This game tests an LLM’s ability to plan and execute valid tile moves to reposition a target tile in a sliding puzzle grid based on adjacency rules.\\
        25 & Bubble Ball Sorting & This game evaluates an LLM’s ability to reason and plan valid moves to sort colored balls into uniform tubes by simulating ball transfers under stacking constraints.\\
        29 & Pipe Game & This game assesses an LLM’s capability to plan and apply spatial transformations by rotating pipes in a grid to create a continuous valid path from start to goal.\\
        38 & Free the Key & This game evaluates an LLM’s ability to reason spatially and sequentially by guiding movable elements to achieve a goal through constrained, rule-based moves.\\
        39 & Map Simulation & This game tests an LLM’s ability to simulate multi-step movement through a dynamic grid while processing complex interactive rules like teleportation, traps, and direction reversals.\\
        40 & Arrow-pathway & This game tests an LLM’s ability to navigate a maze by sequencing directional actions to trigger waypoints in strict order, adapting movements based on both static and dynamic grid constraints.\\
        
        \bottomrule
    \end{tabular}
    }
    \caption{Game Introduction of Spatial and Geometric Reasoning}
    \label{tab:task_Spatial}
\end{table}


==> tables/Strategic_and_Game-Theoretic_Reasoning.tex <==
\begin{table}[h]
    \centering
    \small
    % \renewcommand{\arraystretch}{1.2}
    \resizebox{0.99\textwidth}{!}{
    \begin{tabular}{llp{18cm}}
        \toprule
        No. & Name & Task Content\\
        \midrule
        3  & 2048 & This game tests an LLM's ability to play the 2048 puzzle by choosing the best move (LEFT, RIGHT, UP, or DOWN) based on the current game board to maximize scores through tile merging. \\
        20 & Trust Evolution & This game tests an LLM's ability to identify and exploit opponent behavior patterns through strategic decision-making in repeated prisoner's dilemma scenarios.\\
        21 & N-point & This game tests an LLM’s decision-making ability in a strategic card game, requiring it to balance risk and reward by choosing when to hit or stand based on dynamic thresholds and an opponent's fixed behavior.\\
        31 & Spider Solitaire & This game tests an LLM’s ability to plan and execute strategic moves in Spider Solitaire by evaluating its skill in recognizing valid card sequences, managing limited actions, and achieving the goal of completing full King-to-Ace runs across multiple columns under turn constraints.\\
        34 & Circle the Cat & This game tests an LLM’s spatial reasoning and planning abilities by requiring it to strategically place walls on a hexagonal grid to trap a moving cat before it escapes through an exit.\\
        \bottomrule
    \end{tabular}
    }
    \caption{Game Introduction of Strategic and Game-Theoretic Reasoning}
    \label{tab:task_strategic}
\end{table}


==> tables/Task_intro.tex <==
\begin{table}[h]
    \centering
    \small
    % \renewcommand{\arraystretch}{1.2}
    \resizebox{0.99\textwidth}{!}{
    \begin{tabular}{llp{12cm}p{3cm}}
        \toprule
        No. & Name & Task Content & Ability Dimension\\
        \midrule
        1  & Crossword Puzzle        & This game tests an LLM's date calculation skills by requiring it to deduce the current date based on a future date and a specified number of days between them. & Mathematical and Logical Reasoning \\
        2  & word problem & This game challenges an LLM to find a specific English word that matches given letter and length constraints through logical reasoning. & Language and Textual Reasoning \\
        3  & 2048 & This game tests an LLM's ability to play the 2048 puzzle by choosing the best move (LEFT, RIGHT, UP, or DOWN) based on the current game board to maximize scores through tile merging. &Strategic and Game-Theoretic Reasoning\\
        4 & Sudoku & This game evaluates an LLM's logical reasoning by solving a Sudoku puzzle, ensuring each row, column, and 3x3 block contains the digits 1 to 9 without repetition.&Mathematical and Logical Reasoning \\
        5 & Light Out Game & This game tests an LLM's strategic reasoning by requiring it to switch off all lights on a 3x3 grid through a sequence of toggles that affect each light and its adjacent neighbors. & Mathematical and Logical Reasoning \\
        6 & Minigrid & Based on the Minigrid \citep{MinigridMiniworld23} reinforcement learning system, a control environment tailored for LLMs is constructed, where an agent (ball) performs complex tasks in a partially observable maze, such as picking up items, placing items, avoiding lava, and opening doors. & Control, Interaction, and Task Reasoning \\
        7 & Maze & This game challenges an LLM to find a valid path through a maze from the start point 'I' to the destination 'X', avoiding walls and outputting the sequence of moves. & Spatial and Geometric Reasoning \\
        8 & Sokoban & This game tests an LLM's planning ability by requiring it to solve a Sokoban puzzle, pushing all boxes onto target areas while navigating walls and obeying movement constraints. & Spatial and Geometric Reasoning \\
        \bottomrule
    \end{tabular}
    }
    \caption{XXX}
    \label{tab:task_intro}
\end{table}

